Understanding Layer Significance in LLM Alignment

Aligning large language models (LLMs) through supervised fine-tuning is essential for tailoring them to specific applications. Recent studies suggest that alignment primarily adjusts a model's presentation style rather than its foundational knowledge, indicating that only certain components of the model are significantly impacted. To uncover how alignment affects model behavior at a granular level, we propose identifying which layers within LLMs are most critical to the alignment process. Our approach, named ILA, involves learning a binary mask for the parameter changes in each layer during alignment, as an indicator of layer significance. Experimental results reveal that, despite substantial differences in alignment datasets, the important layers of a model identified by ILA exhibit nearly 90\% overlap, highlighting fundamental patterns in LLM alignment. The results also indicate that freezing non-essential layers improves overall model performance, while selectively tuning the most critical layers significantly enhances fine-tuning efficiency with minimal performance loss. Finally, we discuss how these findings extend from LLM alignment to reasoning.

==> Fig/Fig3_Hyperparameters.tex <==
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.9\linewidth]{Fig/fig1.pdf}
    \caption{The performance of fine-tuning Mistral-7B on the LIMA dataset with the top-$K$ layers frozen, based on the layer importance rankings derived from the No Robots dataset.}
    \label{fig:hyperparameters}
\end{figure}


==> Limitation.tex <==
\section*{Limitations}
This work focuses exclusively on LLM alignment, one of the most critical tasks in LLM applications. We conduct an in-depth investigation into the layer-wise importance ranking during the alignment process across different LLM architectures. However, our algorithm has the potential to extend beyond layer-level analysis. For instance, it could be adapted to neuron-level granularity or applied to other sub-tasks within the broader scope of LLM fine-tuning. These possibilities remain unexplored in this study and offer promising directions for future research.

Moreover, while fine-tuning a subset of parameters can improve alignment performance, this approach may not be the most effective solution for achieving significant performance gains. Alternative strategies, such as increasing the scale and diversity of pretraining datasets or developing more robust and scientifically grounded preference learning methods, could lead to more substantial improvements in alignment. Exploring these avenues would likely provide deeper insights and more effective solutions for optimizing LLM alignment.

==> Table6_Ranking_DiffSeed.tex <==
\begin{table*}[t]
\renewcommand\arraystretch{1.0}
\caption{Jaccard similarities of important layers identified during fine-tuning of \textsc{Llama~\small2}-7B on the LIMA dataset with varying random seeds. The top 75\% highest-scoring layers are designated as important layers.} \label{table:diff_seed}
\centering
\resizebox{0.38\linewidth}{!}{
\begin{tabular}{@{}cccc@{}}
\toprule
Random Seed & seed1 & seed2 & seed3 \\ \midrule
seed1       & -     & -     & -     \\
seed2       & 0.92  & -     & -     \\
seed3       & 0.91  & 0.91  & -     \\ \bottomrule
\end{tabular}
}
\end{table*}

==> Table7_Ranking_DiffStage.tex <==
\begin{table*}[t]
\renewcommand\arraystretch{1.0}
\caption{Jaccard similarities between sets of important layers identified at different milestones during the fine-tuning of \textsc{Llama~\small2}-7B on the LIMA dataset. The top 75\% highest-scoring layers are designated as important layers for this analysis.}\label{table:diff_stage}
% \caption{Jaccard similarity of the important layers when fine-tune \textsc{Llama~\small2}-7B on various datasets. We use the top 75\% highest-scoring layers as important layers.} 
\centering
\resizebox{0.45\linewidth}{!}{
\begin{tabular}{@{}cccccc@{}}
\toprule
\begin{tabular}[c]{@{}c@{}}Training \\ Milestones\end{tabular} & 1\%  & 25\% & 50\% & 75\% & 100\% \\ \midrule
1\%                                                            & -    & -    & -    & -    & -     \\
25\%                                                           & 0.69 & -    & -    & -    & -     \\
50\%                                                           & 0.70 & 0.91 & -    & -    & -     \\
75\%                                                           & 0.69 & 0.90 & 0.92 & -    & -     \\
100\%                                                          & 0.69 & 0.91 & 0.92 & 0.93 & -     \\ \bottomrule
\end{tabular}
}
\end{table*}
